PairPref: When Should Memory Guide the Answer? A Benchmark for Contextual Preference Use

Memory-augmented assistants use retrieved preferences to guide their responses. A small change in the situation can change whether a preference is appropriate while barely affecting its retrieval similarity. Memory benchmarks typically test whether systems store and retrieve preferences, with less attention to when those preferences should apply. We introduce PairPref, a benchmark of contextual preference use. Each pair changes only the situation, keeping the preference, request, and four candidate replies fixed. The preference remains valid in both situations. In the selection track, models must choose the reply that applies the preference only where appropriate. In the free-generation track, they must decide when to apply it without seeing candidate replies. Both tracks use the same 1,227 pairs across 45 preferences and eight situation categories. We evaluate eight models, most of which achieve selection scores ($\Delta$) of 51 to 65 points. In free generation, however, both responses are appropriate for their respective situations in only 3.6\% to 18.3\% of pairs. Models continue to apply the preference in both situations even with fewer retrieved memories, alternative presentation formats, and a stricter prompt. These results show that models still struggle to judge when user preferences apply and respond accordingly.

==> backups/before_related_citations_20260928_143844/02_related_work.tex <==
\section{Related work}
\label{sec:related}
\input{tables/benchmark_protocols}
Preference and memory benchmarks increasingly assess appropriate use as well as recall. Table~\ref{tab:benchmark_protocols} compares their coverage of preference following, suppression, selection, and generation. Appendix~\ref{app:benchmark_comparison} gives evaluation protocols, response formats, dataset sizes, and validation procedures.

\paragraph{Remembering and applying user information.}
Multi-session dialogue tests continuity across chats \citep{xu2022msc}. LoCoMo and LongMemEval evaluate long-term conversational memory; the latter also tests preference questions and abstention when information is unavailable \citep{maharana2024locomo,wu2025longmemeval}. HaluMem localizes failures to extraction, update, and question answering \citep{chen2025halumem}. LaMP and LongLaMP test profile-conditioned classification and long-form generation \citep{salemi2024lamp,kumar2024longlamp}. PrefEval evaluates explicit and implicit preference following through generation and multiple-choice tasks, including response helpfulness \citep{zhao2025prefeval}. PersonaMem tracks evolving user profiles, while CUPID tests inference and application of context-dependent preferences \citep{jiang2025personamem,kim2025cupid}. PairPref holds a preference's validity fixed and tests how its applicability changes with the situation.

\paragraph{Deciding when and how to use memory.}
Benchmarks assess both preference strategies and information-use boundaries. For preference strategies, RPEval evaluates whether preferences should be ignored, support an answer, or dominate it \citep{feng2026rpeval}; BenchPreS measures appropriate application and suppression under formal communication norms \citep{yoon2026benchpres}. For over-personalization and information disclosure, OP-Bench tests irrelevance, sycophancy, and repetition \citep{hu2026opbench}; PersistBench tests leakage and sycophancy alongside beneficial memory use \citep{pulipaka2026persistbench}. CIMemories measures inappropriate disclosure and necessary information coverage \citep{mireshghallah2025cimemories}, while HUSH-Bench tracks sensitive-history use under different memory-access and invitation conditions \citep{xu2026hush}. PairPref isolates a situational reversal within these contextual boundaries: the same still-valid preference and request warrant application in one situation and non-application in another. It evaluates both situations jointly, using fixed candidate replies for selection and the same pairs for free generation. See Appendix~\ref{app:benchmark_distinctions} for details.

\paragraph{Organizing and retrieving memories.}
Memory systems study how records are formed, stored, and retrieved \citep{hu2025memorysurvey}. Generative agents store experiences and reflect on them \citep{park2023generative}. Tiered stores separate short- and long-term records \citep{packer2023memgpt,kang2025memoryos}; linked notes and temporal graphs preserve relations among entries \citep{xu2025amem,rasmussen2025zep}. Retrieval-augmented generation supplies external text \citep{lewis2020rag}, while HippoRAG and its successor use structured retrieval as non-parametric memory \citep{gutierrez2024hipporag,gutierrez2025hipporag2}. Other systems reduce memory-processing costs \citep{chhikara2025mem0,fang2026lightmem} or learn what to write, retrieve, and fuse \citep{yan2026memoryr1,du2025memr3,lu2026fluxmem,zhang2026memgate}. PairPref tests whether models adjust preference use to the situation given fixed memories.


==> backups/before_removing_statements_20260928_154816/statements.tex <==
\subsection*{AI use statement}
Generative AI produced synthetic situations, requests, replies, and companion memories, and performed candidate verification and response scoring. An AI assistant supported manuscript preparation, including language polishing.

\subsection*{Ethics statement}
The benchmark contains synthetic preferences and situations. Two annotators independently assessed revised sample materials (Appendix~\ref{app:human_validation}). A model's social judgments should not become universal behavioral requirements. Situations state constraints explicitly, but interpretation can depend on cultural assumptions. We disclose operational LLM labels and boundaries. Public artifacts must respect licenses and omit identifying metadata.

\subsection*{Reproducibility statement}
Section~\ref{sec:design} describes construction of the 1,227-pair collection; Section~\ref{sec:legacy} describes the dual-track evaluation and exclusions. The supplementary evaluation data, saved judgments, and recomputation scripts support Table~\ref{tab:models}. Appendix~\ref{app:construction_rubric} records construction checks and model configurations, and Appendix~\ref{app:fullreg} provides additional controls.

